Checkpointing algorithms and fault prediction

This paper deals with the impact of fault prediction techniques on checkpointing strategies. We extend the classical first-order analysis of Young and Daly in the presence of a fault prediction system, characterized by its recall and its precision. In this framework, we provide an optimal algorithm to decide when to take predictions into account, and we derive the optimal value of the checkpointing period. These results allow to analytically assess the key parameters that impact the performance of fault predictors at very large scale.

==> pred_not_taken.tex <==
\centering
\begin{tikztimingtable}[
    timing/slope=0,         % no slope
    timing/rowdist=\ttrd,     % row distance
    timing/coldist=2pt,     % column distance
    xscale=3,yscale=1.5, % scale diagrams
    semithick ,              % set line width
  ]


\scriptsize{without failure} & 0.2SG0.5D{\Cr}2S0.5D{\Cr}1.4S G0.6S 0.5D{\Cr}2S0.5D{\Cr}2S0.5D{\Cr}G \\
\scriptsize{with failure} & 0.2SG0.5D{\Cr}2S0.5D{\Cr}1.4S{[red] 0.4D{\D}}{[green] 0.4D{\R}} 2S0.5D{\Cr} 2S 0.5D{\Cr}G \\
\extracode
%  \tableheader{Probability}{\waste}
 \makeatletter
 \begin{pgfonlayer}{background}
%Ligne 0
\arrowtime{0}{12};
\legende{0.7,0}{2}{\T-\Cr};
\legende{3.2,0}{2}{\T-\Cr};
\predfault{4.6,0};
\legende{5.7,0}{2}{\T-\Cr};
\legende{8.2,0}{2}{\T-\Cr};
%Ligne -1
\arrowtime{-\ttrd}{12};
\legende{0.7,-\ttrd}{2}{\T-\Cr};
\legende{3.2,-\ttrd}{1.4}{\Tlost};
\faultbis{4.6,-\ttrd};
\predfault{4.6,-\ttrd};
\legende{5.4,-\ttrd}{2}{\T-\Cr};
\legende{7.9,-\ttrd}{2}{\T-\Cr};

%\draw[color=black] (0.5,2) node {\scriptsize{(b) Prediction not taken into account}};
 \end{pgfonlayer}
\end{tikztimingtable}%


%\centering
%\begin{tikztimingtable}[
%    timing/slope=0,         % no slope
%    timing/coldist=2pt,     % column distance
%    xscale=2.5,yscale=1.5, % scale diagrams
%    semithick ,              % set line width
%  ]


%	& 4D{$\T^{(1)}$}2D{\C}3D{$\T^{(2)}$}                              \\
%$\trust \times (1-\precision)$	& D{$\T^{(1)}$}{[blue,fill=black!20] 2D{\C}} 3D{$\T^{(1)}$}2D{\C} D{ $\T^{(2)}$}    \\
%$\trust \times \precision$  & D{$\T^{(1)}$}{[blue,fill=black!20] 2D{\C}} {[red] D{\D} D{\R}} 3D{$\T^{(1)}$}D{\C}    \\
%$(1-\trust) \times (1-\precision)$	& 4D{$\T^{(1)}$}2D{\C}3D{$\T^{(2)}$}    \\
%$(1-\trust) \times \precision$  & {[red] 3D{$\T^{(1)}$}  D{\D} D{\R}} 4D{$\T^{(1)}$}   \\
%\extracode
%  \tableheader{Probability}{\waste}
% \makeatletter
% \begin{pgfonlayer}{background}
%\predfault{3,1};
%\fault{3,-3};
%\fault{3,-7};
%  % Add background grid lines
%  \begin{scope}[gray,semitransparent,semithick]
%%    \horlines{}
%    \foreach \x in {1,...,8}
%      \draw (\x,1) -- (\x,-8);
%    % similar: \vertlines{1,...,6}
%  \end{scope}
% \end{pgfonlayer}
%\end{tikztimingtable}%


==> pred_taken.tex <==
\centering
\begin{tikztimingtable}[
    timing/slope=0,         % no slope
    timing/rowdist=\ttrd,     % row distance
    timing/coldist=2pt,     % column distance
    xscale=3,yscale=1.5, % scale diagrams
    semithick ,              % set line width
  ]


\scriptsize{without failure} & 0.2SG0.5D{\Cr}2S0.5D{\Cr}0.9S{[fill=black!20] 0.5D{\Cp}} 1.1S 0.5D{\Cr}2S0.5D{\Cr}2S0.5D{\Cr}G \\
\scriptsize{with failure} & 0.2SG0.5D{\Cr}2S0.5D{\Cr}0.9S{[fill=black!20] 0.5D{\Cp}}{[red] 0.4D{\D}}{[green] 0.4D{\R}} 1.1S0.5D{\Cr} 2S 0.5D{\Cr}G \\
\extracode
%  \tableheader{Probability}{\waste}
 \makeatletter
 \begin{pgfonlayer}{background}
%Ligne -1
\arrowtime{0}{12};
\legende{0.7,0}{2}{\T-\Cr};
\legende{3.2,0}{0.9}{\Wregular};
\predfault{4.6,0};
\legende{4.6,0}{1.1}{\T-\Wregular-\Cr};
\legende{6.2,0}{2}{\T-\Cr};
\legende{8.7,0}{2}{\T-\Cr};
%Ligne -2
\arrowtime{-\ttrd}{12};
\legende{0.7,-\ttrd}{2}{\T-\Cr};
\legende{3.2,-\ttrd}{0.9}{\Wregular};
\faultbis{4.6,-\ttrd};
\predfault{4.6,-\ttrd};
\legende{5.4,-\ttrd}{1.1}{\T-\Wregular-\Cr};
\legende{7,-\ttrd}{2}{\T-\Cr};

%\draw[color=black] (0.5,2) node {\scriptsize{(c) Prediction taken into account}};
 \end{pgfonlayer}
\end{tikztimingtable}%


%\centering
%\begin{tikztimingtable}[
%    timing/slope=0,         % no slope
%    timing/coldist=2pt,     % column distance
%    xscale=2.5,yscale=1.5, % scale diagrams
%    semithick ,              % set line width
%  ]


%	& 4D{$\T^{(1)}$}2D{\C}3D{$\T^{(2)}$}                              \\
%$\trust \times (1-\precision)$	& D{$\T^{(1)}$}{[blue,fill=black!20] 2D{\C}} 3D{$\T^{(1)}$}2D{\C} D{ $\T^{(2)}$}    \\
%$\trust \times \precision$  & D{$\T^{(1)}$}{[blue,fill=black!20] 2D{\C}} {[red] D{\D} D{\R}} 3D{$\T^{(1)}$}D{\C}    \\
%$(1-\trust) \times (1-\precision)$	& 4D{$\T^{(1)}$}2D{\C}3D{$\T^{(2)}$}    \\
%$(1-\trust) \times \precision$  & {[red] 3D{$\T^{(1)}$}  D{\D} D{\R}} 4D{$\T^{(1)}$}   \\
%\extracode
%  \tableheader{Probability}{\waste}
% \makeatletter
% \begin{pgfonlayer}{background}
%\predfault{3,1};
%\fault{3,-3};
%\fault{3,-7};
%  % Add background grid lines
%  \begin{scope}[gray,semitransparent,semithick]
%%    \horlines{}
%    \foreach \x in {1,...,8}
%      \draw (\x,1) -- (\x,-8);
%    % similar: \vertlines{1,...,6}
%  \end{scope}
% \end{pgfonlayer}
%\end{tikztimingtable}%

